Simulation Study of a Traffic Light Assistant Based on Vehicle-Infrastructure Communication

Vehicle-infrastructure communication opens up new ways to improve traffic flow efficiency at signalized intersections. In this study, we assume that equipped vehicles can obtain information about switching times of relevant traffic lights in advance, and additionally counting data from upstream detectors. By means of simulation, we investigate, how equipped vehicles can make use of this information to improve traffic flow. Criteria include cycle-averaged capacity, driving comfort, fuel consumption, travel time, and the number of stops. Depending on the overall traffic demand and the penetration rate of equipped vehicles, we generally find several percent of improvement.

==> metadata.tex <==
%-------Data of autors------------------------------------------------
\author{Martin Treiber\footnotemark[1] and Arne Kesting\footnotemark[2] }
\correspondingauthor{Martin Treiber, University of Dresden, Institute
of Traffic Economics, e-mail: treiber@vwi.tu-dresden.de}

%-------Title--------------------------------------------
\title{Simulation Study of a Traffic Light Assistant Based on
Vehicle-Infrastructure Communication}


%-------affiliations----------------------------------
\affiliation{
 \footnotemark University of Dresden\\
 \footnotemark TomTom, Berlin
}								 							 

%--english Keywords--------------------------
\Keywords{Traffic light assistant, intelligent-driver model, adaptive
cruise control, ACC, V2X,
infrastructure-to-vehicle communication}

